Efficient Autoregressive Audio Modeling via Next-Scale Prediction

Audio generation has achieved remarkable progress with the advance of sophisticated generative models, such as diffusion models (DMs) and autoregressive (AR) models. However, due to the naturally significant sequence length of audio, the efficiency of audio generation remains an essential issue to be addressed, especially for AR models that are incorporated in large language models (LLMs). In this paper, we analyze the token length of audio tokenization and propose a novel \textbf{S}cale-level \textbf{A}udio \textbf{T}okenizer (SAT), with improved residual quantization. Based on SAT, a scale-level \textbf{A}coustic \textbf{A}uto\textbf{R}egressive (AAR) modeling framework is further proposed, which shifts the next-token AR prediction to next-scale AR prediction, significantly reducing the training cost and inference time. To validate the effectiveness of the proposed approach, we comprehensively analyze design choices and demonstrate the proposed AAR framework achieves a remarkable \textbf{35}$\times$ faster inference speed and +\textbf{1.33} Fr\'echet Audio Distance (FAD) against baselines on the AudioSet benchmark. Code: \url{https://github.com/qiuk2/AAR}.

==> checklist.tex <==
\section{Checklist}
% Checklist macros
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{teal}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 

This paper:
\begin{itemize}
\item Did you describe the limitations of your work?
\answerYes{YES}
\item Did you discuss any potential risks of your work?
\answerNA{NA}
\item Did you use or create scientific artifacts?
\answerNo{NO}
\item Did you run computational experiments?
\answerYes{YES}
\item Did you report the number of parameters in the models used, the total computational budget (e.g., GPU hours), and computing infrastructure used?
\answerYes{YES}

\item Did you discuss the experimental setup, including hyperparameter search and best-found hyperparameter values?
\answerYes{YES}

\item Did you report descriptive statistics about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run?
\answerYes{YES}

\item If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation, such as NLTK, Spacy, ROUGE, etc.), did you report the implementation, model, and parameter settings used?
\answerYes{YES}

\item Did you use human annotators (e.g., crowdworkers) or research with human participants?
\answerNo{No}

\item Did you use AI assistants (e.g., ChatGPT, Copilot) in your research, coding, or writing?
\answerYes{YES}

\item Did you include information about your use of AI assistants?
\answerNo{No}

\item Elaboration For Yes Or No. For yes, provide a section number. For no, justify why not.
\answerNA{NA}
\end{itemize}

